Towards Developing Safety Assurance Cases for Learning-Enabled Medical Cyber-Physical Systems

Machine Learning (ML) technologies have been increasingly adopted in Medical Cyber-Physical Systems (MCPS) to enable smart healthcare. Assuring the safety and effectiveness of learning-enabled MCPS is challenging, as such systems must account for diverse patient profiles and physiological dynamics and handle operational uncertainties. In this paper, we develop a safety assurance case for ML controllers in learning-enabled MCPS, with an emphasis on establishing confidence in the ML-based predictions. We present the safety assurance case in detail for Artificial Pancreas Systems (APS) as a representative application of learning-enabled MCPS, and provide a detailed analysis by implementing a deep neural network for the prediction in APS. We check the sufficiency of the ML data and analyze the correctness of the ML-based prediction using formal verification. Finally, we outline open research problems based on our experience in this paper.

==> 6_RelatedWork.tex <==
\section{Related Work} \label{sec::relatedWork}
%Besides controller design, APSs have been the subject of the rich literature on hazard identification, hazard prediction, and malfunction detection. The works \cite{meneghetti2019detection,blauw2016review,kolle2019risk,9122567,zhou2021data,zhou2022Robustness} are a few studies to mention. We discuss neither literature on the APS controller design nor the hazard identification as the emphasis of this paper is on designing safety assurance cases for learning-enabled MCPSs, with APSs as a representative example. 
In this section, we discuss the most relevant studies for the purpose of this paper, which is deploying safety assurance cases for learning-enabled MCPS. 
%
In \cite{10.1007/978-3-030-26601-1_12}, Picardi et al. propose an assurance argument pattern to justify the use of ML in clinical diagnosis systems. They consider the application of deep learning in the diagnosis of retinal diseases. They draw a partial safety assurance case for the system to gain insight on how to develop a general pattern. However, the proposed pattern is included in the patterns discussed in \cite{https://doi.org/10.48550/arxiv.2102.01564} by the same authors. In \cite{zhao2021reliability}, Zhao et al. propose an assurance framework for learning-enabled systems. The assurance case starts with probabilistic claims and significantly emphasizes justifying quantitative safety requirements. In the proposed approach, a hazard identification and risk analysis method is used to identify system-level requirements. The requirements are then decomposed into sub-requirements for the system's components and  quantitative metrics are used to express the requirements allocated to the components. To provide evidence, they develop a reliability assessment model concerning the robustness of ML classifiers. However, their proposed framework does not argue over the sufficiency of data. In \cite{klas2021using}, Kl\"{a}s et al. suggest an assurance case that argues over two main claims for ML systems. One of the claims is to achieve a probabilistic target value with a certain level of confidence derived from a quantitative risk acceptance criteria. The second claim is that the risk of AI contributing to a failure is as low as reasonable. The proposed argument is defined over the ML life cycle. However, a concrete example for the proposed approach was not provided. In \cite{10.1145/3453444}, Ashmore et al. define a set of desiderata for each stage of the ML life cycle and review the methods available to address the desiderata. 

In \cite{10.1007/978-3-030-26250-1_30}, Burton et al. attempt to formulate the confidence that an evidence sufficiently supports a performance claim with focus on an automated driving application. For instance, they argue if using a test set, the performance of an ML component passes a threshold, then performance over the entire input space passes a performance threshold. Therefore, the aim is to find such a test set. As defined by the paper, the desideratum is confined to the relevance of data samples. Further, data samples should be capable of detecting faults in ML functions. In \cite{10.1007/978-3-030-83903-1_10}, Burton et al. discuss an approach to assess the assurance of an ML chassis control that estimates the road surface based on sound patterns. A large part of the assurance case design focuses on the ML model itself and less attention is paid to the data used for the development of the model. 
Gauerhof et al. in \cite{10.1007/978-3-030-54549-9_13} concentrate on assessing the safety of a self-driving car when it approaches a pedestrian crossing. The car uses a classifier to detect objects. The authors enumerate the performance and robustness requirements allocated to the ML component, and specify and check the ML data requirements over a dataset.

In \cite{9269875}, Asaadi et al. argue that an assurance case of an autonomous system should be a through-life assurance as ML components of autonomous systems can be updated during runtime by online learning or retraining over new operational data and redeploying into the system. Therefore, the authors propose a methodology in which both dynamic and static elements are considered in the assurance case development. However, the different stages of the ML lifecycle and the key assurance requirements associated with each stage are not considered in this work. 
%
In \cite{8008800}, Calinescu et al. propose a methodology to develop a trustworthy self-adaptive software system in parallel with its associated assurance cases. A partial assurance case is developed at design time where verification and testing are employed to synthesize assurance evidence. This assurance case is completed by further assessment activities and assurance evidence generated at runtime when the system is adapted to a change. This work does not focus on any specific ML applications. On the other hand, the work in \cite{feng_et_al:OASIcs:2014:4526} considers cyber-physical aspects of the system while developing an assurance case. Feng et al. in \cite{feng_et_al:OASIcs:2014:4526} design a safety assurance case for Patient-Controlled Analgesia (PCA) as a case study of MCPS. However, they do not consider the ML contribution to the system design.
